Decoupled-IFTTT: Constraining Privilege in Trigger-Action Platforms for the Internet of Things

Trigger-Action platforms are an emerging class of web-based systems that enable users to create automation rules (or recipes) of the form, "If there is a smoke alarm, then turn off my oven." These platforms stitch together various online services including Internet of Things devices, social networks, and productivity tools by obtaining OAuth tokens on behalf of users. Unfortunately, these platforms also introduce a long-term security risk: If they are compromised, the attacker can misuse the OAuth tokens belonging to millions of users to arbitrarily manipulate their devices and data. In this work, we first quantify the risk users face in the context of If-This-Then-That (IFTTT). We perform the first empirical analysis of the OAuth-based authorization model of IFTTT using semi-automated tools that we built to overcome the challenges of IFTTT's closed source nature and of online service API inconsistencies. We find that 75% of IFTTT's channels, an abstraction of online services, use overprivileged OAuth tokens, increasing risks in the event of a compromise. Even if the OAuth tokens were to be privileged correctly, IFTTT's compromise will not prevent their misuse. Motivated by this empirical analysis, we design and evaluate Decoupled-IFTTT (dIFTTT), the first trigger-action platform where users do not have to give it highly-privileged access to their online services. Our design pushes the notion of fine-grained OAuth tokens to its extreme and ensures that even if the cloud service is controlled by the attacker, it cannot misuse the OAuth tokens to invoke unauthorized actions. Our evaluation establishes that dIFTTT poses modest overhead: it adds less than 15ms of latency to recipe execution time, and reduces throughput by 2.5%.

==> abstract.tex <==
\begin{abstract}
Cloud API integrators are an emerging class of web-based systems that stitch together various
online services such as Internet-connected locks, ovens, and cars as well as services like
Facebook, Google Drive, and Twitter to provide end-users with a simple, yet effective, automation
platform.
These API integrators communicate with various cloud APIs using the popular OAuth protocol,
obtain authorization tokens in the process,
and provide a trigger-action programming abstraction, known as {\em recipes}, for end-users. 
For example, users can set up recipes of the form, ``If my SmartLock is locked, then turn off my oven.''
In this work, we present the first in-depth empirical analysis of the OAuth-based authorization model of If-This-Then-That (IFTTT), a popular
cloud API integrator that integrates with $\totalChannels$ online services and provides more than $200,000$ published recipes.
Performing this analysis is challenging because: (1) IFTTT is closed-source and (2) online service APIs are diverse making large-scale analysis difficult.
We build semi-automated tools to overcome the challenges
and uncover overprivilege as a key security shortcoming of this class of systems. We first characterize the authorization model of $\scrShotChannels$ channels---an abstraction of online service APIs---for which we could record authorization sessions that consist of the OAuth authorization 
URL and a screenshot of the permissions prompt. 
Our analysis reveals that $\channelsNoControl$ of the time, users are 
only presented with an all-or-nothing choice while authorizing IFTTT channels and $83\%$ of online services do not provide
fine-grained scoping for IFTTT authorizations. We then perform an in-depth overprivilege analysis on channels' integration
with online service APIs. Out of a total of $\measurableChannelsAll$ channels that have publicly documented APIs from our
set of $\scrShotChannels$ channels, we analyze $\numApisStudied$ APIs across $\numChannelsStudiedAll$ channels, including 
all $\numChannelsStudiedIoT$ cyber-physical
channels, and find that $\overprivdChannelsAll$ channels have access to online service APIs that they do {\em not} need
to implement their triggers and actions. Our in-depth analysis covers $\recipeCoverageTrigger$ of all recipes involved
in the set of $\measurableChannelsAll$ channels that can be studied in-depth.
Overprivileged access to channels increases privacy, security, and safety risks. For example, using the overprivileged access of the popular 
Particle channel for interacting with physical devices, we were able to reprogram a Particle chip's firmware by using a single HTTP API call.


%Cloud API integrators are an emerging class of web-based systems that stitch together various
%online services to provide a simple, yet effective, automation platform. 

%These API integrators communicate with various cloud APIs using the popular OAuth protocol,
%obtain authorization tokens in the process,
%and provide a trigger-action programming abstraction, known as {\em recipes}, for end-users. 

%Furthermore, due to the current trend in connecting cyber-physical devices to the Internet, we observe
%that such cloud API integrators are evolving to support automation of physical devices such as smart locks and ovens.


%We examine the integration of IFTTT with these services by analyzing the authorization transaction of $\scrShotChannels$ channels and examining $\numApisStudied$ APIs in-depth across $\numChannelsStudiedAll/\measurableChannelsAll$ services that provide access to their APIs. This leads us to a coverage of $\recipeCoverageTrigger$ across all measurable trigger-action
%combinations.
%Our research uncovers overprivilege as the main security shortcoming of this class of systems and examines the design flaws and 
%trade-offs that lead to it.
%IFTTT and the online services it integrates with are closed-source, making our measurements challenging. We overcame the challenges using a novel combination of techniques including downgrade attacks and scope reuse to build a semi-automated measurement pipeline. 

%Our results show that $\channelsNoControl$ of the online services that correspond to IFTTT channels do not provide users with any 
%control over data that is being shared and $\channelsNotDescriptive$ of them do not provide explanation for types of access they seek. 
%Furthermore, $75\%$ of the channels we studied in-depth provide IFTTT with overprivileged access to their APIs. 

%This overprivilege
%increases the risk a user faces. For example, using the overprivileged access of the Particle channel, we were able to reprogram
%a Particle chip's firmware using a single HTTP API call.

\end{abstract}


==> appc.tex <==
\section*{Appendix C}
\label{sec:appc}
We show example screenshots for our characterization of $\scrShotChannels$ channels. Figure~\ref{fig:scrfb} shows that Facebook is only one of
 $\fineOAuth$ online services that provide the user with fine-grained control over scopes that are granted to IFTTT. 
Figure~\ref{fig:scrfiverr} shows an example online service, Fiverr, that explains the level of privilege being requested. It does not provide
the user the ability to modify the request. Figure~\ref{fig:scrshot2} provides a comparison of the levels of descriptions
that online services provide to users when IFTTT requests authorization.



   \begin{figure*}[!tb]
   	\centering
   	\includegraphics[width=.8\textwidth]{figs/linkedin.png}
   	\caption{Linkedin does not provide user with any control over what data is being shared, but allows the user to select an access duration for the token.}
   	\label{fig:scrlinkedin}
   \end{figure*}

\begin{figure*}[!tb]
 \center
     \begin{subfigure}[t]{0.49\textwidth}
       \centering
       \vspace{-13.6em}
       \includegraphics[width=\columnwidth]{figs/rainmachine.png}  
       \caption{\textbf{RainMachine (Non-descriptive)}}
       \label{fig:scrrainmachine}
       
       \includegraphics[width=\columnwidth]{figs/tumblr.png}
       \caption{\textbf{Tumbler (Semi-descriptive)}}
       \label{fig:scrtumblr}
     \end{subfigure}
   ~ 
   \begin{subfigure}[t]{0.49\textwidth}
     \centering
     \includegraphics[width=\columnwidth]{figs/twitter.png}
     \caption{\textbf{Twitter (Descriptive)}}
     \label{fig:scrtwiter}
   \end{subfigure}
   
   \caption{A comparison of different levels of description provided to users. While $59\%$ of online services provide descriptive information on the token's privileges similar to Twitter (\ref{fig:scrtwiter}), other services either provide inadequate information (\eg Tumbler, \ref{fig:scrtumblr}) or no information (\eg RainMachine, \ref{fig:scrrainmachine}).}

\label{fig:scrshot2}
\end{figure*}



==> attacks.tex <==
\section{Exploiting Design Vulnerabilities}
\label{sec:attacks}
\ef{not sure whether we need this attack since I am explaining the negative implications of overpriv with case studies in III.E}
Describe the two types of attack. present our evaluation on number of suceptable channels and links. 

\subsection{Downgrade Attack}

\subsection{Downgrade with Redirect Attack}

\subsection{Implications}
Discuss that these attacks were only samples showing the possibility. these systems are high value targets. Lack of Authenticity verification causes these systems to be vulnerable to any attacks on OAuth


==> casestudy.tex <==
\section{Case Study}
show how we compute the overprivilege so that they don't attack us.

the following section is simply a discussion of how we automated/scaled up the measurement, and what are the overall results.

and the challenges we faced while scaling up

==> disclosure.tex <==
%	\begin{figure*}[!b]
%		\centering
%		\includegraphics[width=.8\textwidth]{figs/facebook.png}
%		\caption{Facebook is one of only $\fineOAuth$ online services that provide the user with fine-grained control over privilege that is granted to the OAuth token.}
%		\label{fig:scrfb}
%	\end{figure*}
%	
%	   \begin{figure*}[!tb]
%	   	\centering
%	   	\includegraphics[width=.8\textwidth]{figs/fiverr.png}
%	   	\caption{Although the Fiverr online service notifies the user of the level of privilege that is being requested, it does not provide the user with the ability to modify the permissions being requested.}
%	   	\label{fig:scrfiverr}
%	   \end{figure*}
	   

\section*{Responsible Disclosure}
We initiated communication with IFTTT regarding our overprivilege results. They responded to us on Sep 14th, 2016 saying that the API team will be looking into the issue. We have not heard back from them since.

%We will also forgo releasing our dataset until fixes have been made to the system and affected channels.


==> prior_reviews.tex <==
\section*{Summary of Differences from NDSS 2017 Submission}
In our original NDSS submission, we focused on the problem of over-privilege in trigger-action platforms. Although we hinted at various approaches that could be used to protect these systems, we did not include design or evaluation of such a solution. The reviews we received suggested this to be the main shortcoming of our work. In this submission, we condensed our measurement results to section~\ref{sec:empirical} and moved some of the additional evaluations to the Appendix. Next, we distilled the lessons we learned based on our study in section~\ref{sec:lessons} and discussed an appropriate threat model for trigger-action platforms. Using these lessons and model, we designed, built, and evaluated \longsys, a trigger-action platform that tackles the over-privilege problem by enabling end-to-end integrity of recipes execution. Our design uses fine-grained OAuth tokens and ensures that tokens can not be used for any recipe other than the one they were issued for. We evaluate factors such as storage, transmission size, and latency overhead in our system and compare it to the existing trigger-action platforms design. 


\section*{Prior Reviews}
We have reproduced the reviews that we received from NDSS 2017 below

\noindent{\textbf{Review 1.}}

       Overall merit: 2. Weak reject
       
                 Reviewer expertise: 3. Knowledgeable

                         ===== Paper summary =====

The paper analyses the authorization model of IFTTT, or more precisely looks at how the 128 channels implement OAuth to grant privileged access to their APIs. The authors find some egregious instances of overprivilege, but more generally find that most channels could improve their permission granularity, descriptions of behavior, or implementation of OAuth scoping.

                        ===== Paper Strengths =====

* Clever use of OAuth hacks to map out API functions
* Large scale IFTTT recipe analysis
* First security analysis of IFTTT

                       ===== Paper weaknesses =====

* Identified problems are known problems with OAuth
* Solutions are not well thought out or evaluated

                ===== Additional comments for author =====

I was excited to read this paper since I believe that important to understand how emerging technologies are being used to inform the design of security systems for these technologies. This paper does a great job of mapping out the problem space, but ends abruptly without analyzing whether the proposed solutions make sense or are feasible. The paper starts out by saying that the results and lessons learned can help in the design of other systems, but fails to concretely demonstrate this part. It would be more helpful to the reader to see the solutions analyzed in more depth in the last 2 pages instead of the giant screenshots in the appendix.

I was also underwhelmed by the long-term research takeaways from the paper. The 2 pages dedicated to examples of OAuth misuses by different services is anecdotally interesting, but will become obsolete once/if the services fix those issues. Further, it seems like the main problems identified resemble problems in other permission-based domains (granularity of permissions, usability problems).  We know OAuth has limitations, we known developers don’t implement it with a focus on security, and IFTTT is just a place where all these errors are concentrated.

The solutions proposed (sec IV) are easy to suggest but could be difficult to implement. For example, the “one token per recipe” strategy sounds good in theory, but would require more user approvals. Going entirely “least privilege” might result in an explosion of permissions… Actually most of the content in sec IV is not unique to IFTTT, but rather are common defenses against (OAuth) overprivilege.

As a minor issue, the measurement pipeline is described as being “semi-automated”, but from reading the details it appears to require substantial manual input, analysis, and curation. While I appreciate the effort in building this, I’m not sure this analysis would be easily applicable to other API integrators.

\noindent{\textbf{Review 2.}}


                      Overall merit: 2. Weak reject
                      
                      
                 Reviewer expertise: 4. Expert


                         ===== Paper summary =====

The authors present an empirical study of how the "cloud API
integrator" IFTTT makes use of its permissions on third party
websites. While the main focus is on "overprivilege", i.e., IFTTT
requesting access to API functions that it does not need, the authors
also present some other statistics collected during the analysis.

                        ===== Paper Strengths =====

The paper is very well-written, an easy read, and methodology and
results are made clear.  A useful running example explains IFTTT's
mechanisms.

The results make clear that the authors were able to identify a
widespread problem in the IFTTT cloud API integrator (although not a
severe one, see below).

                       ===== Paper weaknesses =====

Altogether, the scientific contribution of this paper is very limited.

- The outcome of the paper seems not really surprising. Also, it is
  not a fundamental problem: First, it only affects users of IFTTT and
  similar services. Second, the consequences are not severe. Of
  course, it would be better and more secure if IFTTT and other
  platforms would request the smallest amount of privileges possible.

- The paper focuses on IFTTT only. IFTTT is the biggest (and as far as
  I know) the first cloud integrator platform. Focussing on IFTTT is
  fine for an initial study in this area, but it also limits the
  impact of the paper somewhat.

- One kind of overprivilege criticized by the authors occurs when a
  user's recipes do not use all triggers or actions of some channel.
  This, however, is understandable from a usability point of view:
  Re-requesting a user's permission each time the user starts using a
  new trigger or action would be annoying.

                ===== Additional comments for author =====

The attack described as the "open redirector" attack is, strictly
speaking, not the open redirector attack. Instead, it is just bad
checking of the redirect URIs in OAuth implementations. The open
redirector attack is based on a URI that redirects users to arbitrary
websites, which can then be used to redirect OAuth response data. 

The authors further criticize that there are channels where users have
only a binary choice of accepting or denying access to all API
functions (binary choice). It is not so clear, however, (a) how many
of these channels requested only a single permission, leaving a binary
choice as the only sensible user interface, and (b) how many channels
requested permissions that would not work without other permissions,
ruling out a finer-grained choice for the user.


